Differentiable Modeling of Planet and Substellar Atmosphere: High-Resolution Emission, Transmission, and Reflection Spectroscopy with ExoJAX2

Modeling based on differentiable programming holds great promise for astronomy, enabling advanced techniques such as gradient-based posterior sampling and optimization. This paradigm motivated us to develop ExoJAX (Kawahara et al. 2022), the first auto-differentiable spectrum model of exoplanets and brown dwarfs. ExoJAX directly calculates cross-sections as functions of temperature and pressure to minimize interpolation errors in high-dispersion spectra, although initial work focused on narrowband emission spectroscopy. Here, we introduce a fast, memory-efficient opacity algorithm and differentiable radiative transfer for emission, transmission, and reflection spectroscopy. In the era of data-rich JWST observations, retrieval analyses are often forced to bin high-resolution spectra due to computational bottlenecks. The new algorithm efficiently handles native-resolution data, preserving the full information content and dynamic range. The advances proposed in this paper enable broader applications, demonstrated by retrievals of GL229 B's high-dispersion emission, WASP-39 b's JWST mid-resolution transmission at original resolution (R $\sim$ 2,700), and Jupiter's reflection spectrum. We derive a C/O ratio for GL229 B consistent with its host star, constrain WASP-39 b's radial velocity from molecular line structures, and infer Jupiter's metallicity in line with previous estimates.

==> name.tex <==
    gamma vald3 & Uses van der Waals gamma from line lists (VALD or Kurucz) or estimates from \cite{1955psmb.book.....U}. \\
    gamma uns & Approximated gamma based on \cite{1955psmb.book.....U}. \\
    gamma KA3 & Derived from the third equation in \cite{1981SAOSR.391.....K} (page 4). \\
    gamma KA4 & From the fourth equation in \cite{1981SAOSR.391.....K} (page 4). \\
    gamma KA3s & As gamma KA3, but without differentiating iron group elements. \\
    \hline
